Search for lepton-flavor-violating $\tau^- \to \ell^- K_s^0$ decays at Belle and Belle II

We present the results of a search for charged-lepton-flavor violating decays $\tau^{-} \rightarrow \ell^{-}K_{S}^{0}$, where $\ell^{-}$ is either an electron or a muon. We combine $e^+e^-$ data samples recorded by the Belle II experiment at the SuperKEKB collider (428 fb$^{-1}$) with samples recorded by the Belle experiment at the KEKB collider (980 fb$^{-1}$) to obtain a sample of 1.3 billion $e^+e^-\to\tau^+\tau^-$ events. We observe 0 and 1 events and set $90\%$ confidence level upper limits of $0.8 \times 10^{-8}$ and $1.2 \times 10^{-8}$ on the branching fractions of the decay modes $\tau^{-} \rightarrow e^{-}K_{S}^{0}$ and $\tau^{-} \rightarrow \mu^{-}K_{S}^{0}$, respectively. These are the most stringent upper limits to date.

==> 031-cutbased.tex <==
%\begin{itemize}
    %\item tag 
    %\item BG rejection
    %\item eff. 
    %\item number of estimated BG events
    %\item validation
%\end{itemize}

We require that the \emph{tag} hemisphere contains only one charged particle. Consequently, the event is reconstructed by requiring exactly four charged particles with zero total charge. Within the tag side, we categorize the charged particle as either a lepton (targeting the $\tau^+ \to e^+ \nu_e \bar\nu_\tau$ or $\tau^+ \to \mu^+ \nu_\mu \bar\nu_\tau$ decays) or a hadron (correspondingly, the $\tau^+\to h^+ n \pi^0 \bar\nu_\tau$ decays). No restrictions are placed on the energy or the number of neutral particles. 

The signal region is defined taking into account the correlation between the \Mmu{} and \dE. The resolutions  $\delta_{\Mmu^\prime }$ and $\delta_{\dE^\prime }$ of the uncorrelated quantities, $\Mmu^\prime$ and $\dE^\prime$ are estimated in a fit 
using a combination of two Cristal Ball and a Gaussian functions. We use the intervals $-10 \delta_{\Mmu^\prime } < \Mmu^\prime < 5 \delta_{\Mmu^\prime }$ and $-10 \delta_{\dE^\prime } < \dE^\prime < 5 \delta_{\dE^\prime }$ around the mean values of $\Mmu^\prime$  and $\dE^\prime$  as signal region. 

The backgroung suppression is performed in the extended signal region defined as $\pm 10\delta$. The main background contamination originates from \eetautau, \eemumumumu and \eeqqbar events. %using 2.5M simulated signal events and 5\invab of \eetautau, \eemumumumu and \eeqqbar events.  
The contamination from $\epem \to \epem nh$ events is mitigated using data-driven requirements $0.4<\theta_{p_{\rm{miss}}}^*<2.7$\rad for leptonic and $0.3<\theta_{p_{\rm{miss}}}^*<2.8$\rad for hadronic tags, along with a limit of only one signal track pointing to the endcaps. 
These requirements suppress also the $\epem \to \ell^+\ell^-\ell^+\ell^-$ and $\epem \to e^+e^-h^+h^-$, which are further rejected requiring $\Delta E_{\tau_{\rm tag}}<-0.8$\gev. 
The \eeqqbar and \eetautau events are suppressed requiring $\visE<10.2$\gev, $0.90 < T< 0.97$, and $p_{\rm{miss}}^*>0.4$\gevc. 
%remaining background from \qqbar and \eetautau are suppressed by
%, while requirements on the missing momentum of the event $p_{\rm{miss}}^*>$0.4, its corresponding polar angle 0.3$<\theta_{p_{\rm{miss}}}^*<$2.8\rad and on the number of signal tracks pointing to the endcaps to be less than two are intended to reject the processes not taken into account in the simulated samples. 
%a  and ((trackI_3prong_theta>0.4 and trackII_3prong_theta>0.4) or (trackI_3prong_theta>0.4 and trackIII_3prong_theta>0.4) or (trackII_3prong_theta>0.4 and trackIII_3prong_theta>0.4))
To further suppress the remaining background events, strict requirements for the muon identification are imporsed on the tracks in the signal side. 
We separate the tracks according to their momentum in three categoris : $p < 0.7$\gevc, $0.7<p<1.0$\gevc, and $p>1$\gevc. 
%%%This choice follows the muonID efficiencies behaviour, dominated by how much the KLM detector is exploited. 
The requirements on the discriminator $P_\mu$ are optimised using the Punzi figure-of-merit~\cite{Punzi:2003bu} defined as 
\begin{equation}
    {\rm FOM_{Punzi}} =\frac{\varepsilon_{\textit{sig}}}{\alpha / 2 + \sqrt{N_{BG}}} .
\end{equation}
Here $\varepsilon_{\textit{sig}}$ is the signal efficiency, $\alpha$ is chosen to be 1.28, corresponding to the 90\% of C.L., and N$_{BG}$ is the number of background. % events that survive the selection. 
The resulting requirements for tracks in momentum ranges $p < 0.7$\gevc, $0.7<p<1.0$\gevc and $p>1$\gevc are $P_\mu >0.95$, $P_\mu >0.55$ and $P_\mu >0.9$ , respectively, for leptonic-tag events. The corresponding requirements for the hadronic-tag events are $P_\mu >0.75$, $P_\mu >0.9$, and $P_\mu >0.95$. 
% A cut on the momentum of signal side tracks to be greater than 0.2\gevcc is applied to remove uncovered regions of muonID 
%$\mathcal{L}_\mu$ 
%corrections. 
%variables is considered by correcting the simulation with dedicated correction factors. These corrections are missing for tracks with momentum less than 0.2\gev. 
%trackI_3prong_p>0.2 and trackII_3prong_p>0.2 and trackIII_3prong_p>0.2
%For tracks in the leptonic (hadronic) tag with $p< 0.7$\gevc we applied $P-\mu >0.95$ (0.75), with 0.7$<$p$<$1.0\gevcc larger than 0.55 (0.9) while for p$>$1\gevcc larger than 0.9 (0.95).

%In fact, for example, tracks with p<0.7GeV does not reach the KLM.
%Then, we vary the muonID requirement on these tracks between 0.5 and 1, in steps of 0.05, and we pick the combination of cuts that provides the highest FOM value.
%Results provide cuts on muonID$>$0.95 on tracks falling in r1 and r3 ranges and muonID$>$0.90 for those in r2. 

Independent simulated samples %of 2.5M signal and 3\invab 
of $\epem \to \qqbar$ and \eetautau events are used to estimate the efficiency of the signal \taumu events and the number of background events expected in the signal region. 
%
Since the estimation of the number of expected events in the signal region relies on the simulation, the agreement of the experimental and simulated data is verified in the regions $\pm 40$ widths away from the signal region and in the signal region by substituted the muon identification requirements with the ones of the pion identification. In the latter, we observe an overestimation of the \qqbar contribution. By applying a correction, we reach a good agreement between experimental and simulated data in the region $\pm 40$ widths away from the signal region. The same correction is applied also for the estimation of the number of expected background events in the signal region.  
%
%A good agreement between experimental and simulated data is observed in the first case, and an overestimation of the \qqbar contribution in the second. 
The signal efficiency is found to be  14.94\%, with $7.79\%$ and $7.15\%$ corresponding to leptonic and hadronic tags, respectively. The signal efficincy is nearly twice larger than what was achieved at first generation $B$-factory experiments. The number of expected background events is 0.43 for \lumi\invfb. 



%The latter is the correspondingto an integrated luminosity of 424\invfb and includes all the data/simulation correction sources described in this paper. 
%The number of expected events in the signal region to be used for the limit extraction come from the selection defined in Section~\ref{sec:optimisation}, and it is validated using both control channel and sideband approaches. 
%We use the $\tau^- \to \pi^-\pi^+\pi^-\nu$ control channel where we substituted the muonID requirements with the pion identification ones, with corresponding data/simulation corrections applied. 
%The remaining analysis requirements are applied to the control channel without any modifications. 
%The observed data/simulation discrepancy is attributed to a \qqbar overestimated cross section in the {\belletwo{}} simulation. Thus, we extract a correction factor to be applied to the \qqbar background in the main analysis. 
%This correction is also applied during the Side-Band (SB) checks. We followed a blinded strategy, therefore we look outside the SR up to 40 widths, as defined in Section~\ref{sec:oneprong}, {\color{red} where the data and MC entries are in agreement.}
%

==> Makefile <==
# input files
SOURCES:=title.tex abstract.tex pacs.tex body.tex authors.tex material.tex acknowledgements.tex \
         definitions.tex references.bib instructions.tex belle2-symbols.tex belle2.bst $(wildcard figures/*)

# default is note
note: note.tex $(SOURCES)
	latexmk -pdf -bibtex note

# tarball
%.paper: %.tex $(SOURCES)
	@./create_paper $@

# latex build
%: %.tex $(SOURCES)
	latexmk -pdf -bibtex $@

# removes temporary files
.PHONY : clean
clean:
	@rm -f *~ *.toc *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *prlNotes.bib *.fdb_latexmk *.fls

# make word count
prlcount: 
	sed 's/{wordcount}{false}/{wordcount}{true}/' prl.tex > prl-count.tex
	$(prl-count)
	chmod +x wordcount.sh
	./wordcount.sh prl-count
	@rm wordcount.pdf prl-count*
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo ''
	@echo 'Abstracts should also be ≤ 600 characters'


==> addref <==
#!/usr/bin/env python3
# -*- coding: utf-8 -*-

from urllib.request import urlopen
import sys
import re

# check arguments
if len(sys.argv) != 2:
    print('ERROR: An arXiv or inspire ID has to be given as argument')
    sys.exit(1)

id = sys.argv[1]
bibfile = 'references.bib'

# get bibtex from inspire
if '/' in id:
    query = 'eprint'
elif '.' in id:
    query = 'arxiv'
else:
    query = 'recid'
try:
    bibtex = urlopen(f'https://inspirehep.net/api/literature?q={query}%3A{id}&format=bibtex').read().decode()
except:
    print(f'ERROR: Query for {id} failed.')
    sys.exit(1)
if len(bibtex) == 0:
    print(f'ERROR: Could not get bibtex for {id}.')
    sys.exit(1)

# check whether the entry is already in references.bib
entry = re.compile('@[\w]*{([\S]*),').findall(bibtex)[0]
with open(bibfile) as bib:
    if entry in bib.read():
        print(f'ERROR: {bibfile} already contains the entry {entry}.')
        sys.exit(1)

# add bibtex to references.bib
with open(bibfile, 'a+') as bib:
    bib.write('\n' + bibtex)

print(f'Entry {entry} added to {bibfile} -> \\cite{{{entry}}}')


==> belle2-symbols.tex <==
% A. Di Canto (16-Sep-2022)
% Based on:
%  - babarsym.tex (by D. Hitlin, D. MacFarlane, P. Dauncey, R. Waldi)
%  - lhcb-symbols-def.tex (by U. Egede, T. Skwarnicki, C. Parkes, R. Oldeman, P. Koppenburg)

\RequirePackage{xspace}
\RequirePackage{relsize}

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\belletwo{\mbox{Belle~II}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\lhcb {\mbox{LHCb}\xspace}
%\def\babar  {\mbox{BaBar}\xspace}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

%%%%%%%%%%%%%
% Particles
%%%%%%%%%%%%%
\def\Palpha      {\ensuremath{\alpha}\xspace}
\def\Pbeta       {\ensuremath{\beta}\xspace}
\def\Pgamma      {\ensuremath{\gamma}\xspace}                 
\def\Pdelta      {\ensuremath{\delta}\xspace}                 
\def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
\def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
\def\Pzeta       {\ensuremath{\zeta}\xspace}                 
\def\Peta        {\ensuremath{\eta}\xspace}                 
\def\Ptheta      {\ensuremath{\theta}\xspace}                 
\def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
\def\Piota       {\ensuremath{\iota}\xspace}                 
\def\Pkappa      {\ensuremath{\kappa}\xspace}                 
\def\Plambda     {\ensuremath{\lambda}\xspace}                 
\def\Pmu         {\ensuremath{\mu}\xspace}                 
\def\Pnu         {\ensuremath{\nu}\xspace}                 
\def\Pxi         {\ensuremath{\xi}\xspace}                 
\def\Ppi         {\ensuremath{\pi}\xspace}                 
\def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
\def\Prho        {\ensuremath{\rho}\xspace}                 
\def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
\def\Ptau        {\ensuremath{\tau}\xspace}                 
\def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
\def\Pphi        {\ensuremath{\phi}\xspace}                 
\def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
\def\Pchi        {\ensuremath{\chi}\xspace}                 
\def\Ppsi        {\ensuremath{\psi}\xspace}                 
\def\Pomega      {\ensuremath{\omega}\xspace}                 
\mathchardef\PDelta="7101
\mathchardef\PXi="7104
\mathchardef\PLambda="7103
\mathchardef\PSigma="7106
\mathchardef\POmega="710A
\mathchardef\PUpsilon="7107
\def\PA      {\ensuremath{A}\xspace}                 
\def\PB      {\ensuremath{B}\xspace}                 
\def\PC      {\ensuremath{C}\xspace}                 
\def\PD      {\ensuremath{D}\xspace}                 
\def\PE      {\ensuremath{E}\xspace}                 
\def\PF      {\ensuremath{F}\xspace}                 
\def\PG      {\ensuremath{G}\xspace}                 
\def\PH      {\ensuremath{H}\xspace}                 
\def\PI      {\ensuremath{I}\xspace}                 
\def\PJ      {\ensuremath{J}\xspace}                 
\def\PK      {\ensuremath{K}\xspace}                 
\def\PL      {\ensuremath{L}\xspace}                 
\def\PM      {\ensuremath{M}\xspace}                 
\def\PN      {\ensuremath{N}\xspace}                 
\def\PO      {\ensuremath{O}\xspace}                 
\def\PP      {\ensuremath{P}\xspace}                 
\def\PQ      {\ensuremath{Q}\xspace}                 
\def\PR      {\ensuremath{R}\xspace}                 
\def\PS      {\ensuremath{S}\xspace}                 
\def\PT      {\ensuremath{T}\xspace}                 
\def\PU      {\ensuremath{U}\xspace}                 
\def\PV      {\ensuremath{V}\xspace}                 
\def\PW      {\ensuremath{W}\xspace}                 
\def\PX      {\ensuremath{X}\xspace}                 
\def\PY      {\ensuremath{Y}\xspace}                 
\def\PZ      {\ensuremath{Z}\xspace}                 
\def\Pa      {\ensuremath{a}\xspace}                 
\def\Pb      {\ensuremath{b}\xspace}                 
\def\Pc      {\ensuremath{c}\xspace}                 
\def\Pd      {\ensuremath{d}\xspace}                 
\def\Pe      {\ensuremath{e}\xspace}                 
\def\Pf      {\ensuremath{f}\xspace}                 
\def\Pg      {\ensuremath{g}\xspace}                 
\def\Ph      {\ensuremath{h}\xspace}                 
\def\Pi      {\ensuremath{i}\xspace}                 
\def\Pj      {\ensuremath{j}\xspace}                 
\def\Pk      {\ensuremath{k}\xspace}                 
\def\Pl      {\ensuremath{l}\xspace}                 
\def\Pm      {\ensuremath{m}\xspace}                 
\def\Pn      {\ensuremath{n}\xspace}                 
\def\Po      {\ensuremath{o}\xspace}                 
\def\Pp      {\ensuremath{p}\xspace}                 
\def\Pq      {\ensuremath{q}\xspace}                 
\def\Pr      {\ensuremath{r}\xspace}                 
\def\Ps      {\ensuremath{s}\xspace}                 
\def\Pt      {\ensuremath{t}\xspace}                 
\def\Pu      {\ensuremath{u}\xspace}                 
\def\Pv      {\ensuremath{v}\xspace}                 
\def\Pw      {\ensuremath{w}\xspace}                 
\def\Px      {\ensuremath{x}\xspace}                 
\def\Py      {\ensuremath{y}\xspace}                 
\def\Pz      {\ensuremath{z}\xspace}                 

%% generic

\def\hpm  {\ensuremath{\Ph^\pm}\xspace} 
\def\hp     {\ensuremath{\Ph^+}\xspace} 
\def\hm    {\ensuremath{\Ph^-}\xspace}
\def\ellpm{\ensuremath{\ell^\pm}\xspace}
\def\ellp   {\ensuremath{\ell^+}\xspace}
\def\ellm  {\ensuremath{\ell^-}\xspace}

%% Leptons

\let\emi\en
\def\electron   {\ensuremath{\Pe}\xspace}
\def\en         {\ensuremath{\Pe^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{\Pe^+}\xspace}
\def\epm        {\ensuremath{\Pe^\pm}\xspace} 
\def\epem       {\ensuremath{\Pe^+\Pe^-}\xspace}
\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\mmu        {\ensuremath{\Pmu}\xspace}
\def\mup        {\ensuremath{\Pmu^+}\xspace}
\def\mun        {\ensuremath{\Pmu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\Pmu^+\Pmu^-}\xspace}
\def\mtau       {\ensuremath{\Ptau}\xspace}

\def\taup       {\ensuremath{\Ptau^+}\xspace}
\def\taum       {\ensuremath{\Ptau^-}\xspace}
\def\tautau     {\ensuremath{\Ptau^+\Ptau^-}\xspace}

\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {\ensuremath{\Pnu}\xspace}
\def\neub       {\ensuremath{\overline{\Pnu}}\xspace}
\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {\ensuremath{\neu_e}\xspace}
\def\neueb      {\ensuremath{\neub_e}\xspace}
\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {\ensuremath{\neu_\mu}\xspace}
\def\neumb      {\ensuremath{\neub_\mu}\xspace}
\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {\ensuremath{\neu_\tau}\xspace}
\def\neutb      {\ensuremath{\neub_\tau}\xspace}
\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {\ensuremath{\neu_\ell}\xspace}
\def\neulb      {\ensuremath{\neub_\ell}\xspace}
\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {\ensuremath{\Pgamma}\xspace}
\def\H      {\ensuremath{\PH^0}\xspace}
\def\Hp     {\ensuremath{\PH^+}\xspace}
\def\Hm     {\ensuremath{\PH^-}\xspace}
\def\Hpm    {\ensuremath{\PH^\pm}\xspace}
\def\W      {\ensuremath{\PW}\xspace}
\def\Wp     {\ensuremath{\PW^+}\xspace}
\def\Wm     {\ensuremath{\PW^-}\xspace}
\def\Wpm    {\ensuremath{\PW^\pm}\xspace}
\def\Z      {\ensuremath{\PZ^0}\xspace}

%% Quarks

\def\quark     {\ensuremath{\Pq}\xspace}
\def\quarkbar  {\ensuremath{\overline \quark}\xspace}
\def\qqbar     {\ensuremath{\quark\quarkbar}\xspace}
\def\uquark    {\ensuremath{\Pu}\xspace}
\def\uquarkbar {\ensuremath{\overline \uquark}\xspace}
\def\uubar     {\ensuremath{\uquark\uquarkbar}\xspace}
\def\dquark    {\ensuremath{\Pd}\xspace}
\def\dquarkbar {\ensuremath{\overline \dquark}\xspace}
\def\ddbar     {\ensuremath{\dquark\dquarkbar}\xspace}
\def\squark    {\ensuremath{\Ps}\xspace}
\def\squarkbar {\ensuremath{\overline \squark}\xspace}
\def\ssbar     {\ensuremath{\squark\squarkbar}\xspace}
\def\cquark    {\ensuremath{\Pc}\xspace}
\def\cquarkbar {\ensuremath{\overline \cquark}\xspace}
\def\ccbar     {\ensuremath{\cquark\cquarkbar}\xspace}
\def\bquark    {\ensuremath{\Pb}\xspace}
\def\bquarkbar {\ensuremath{\overline \bquark}\xspace}
\def\bbbar     {\ensuremath{\bquark\bquarkbar}\xspace}
\def\tquark    {\ensuremath{\Pt}\xspace}
\def\tquarkbar {\ensuremath{\overline \tquark}\xspace}
\def\ttbar     {\ensuremath{\tquark\tquarkbar}\xspace}

%% Light mesons

\def\pion  {\ensuremath{\Ppi}\xspace}
\def\piz   {\ensuremath{\pion^0}\xspace}
\def\pizs  {\ensuremath{\pion^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pion^0\pion^0}\xspace}
\def\pip   {\ensuremath{\pion^+}\xspace}
\def\pim   {\ensuremath{\pion^-}\xspace}
\def\pipi  {\ensuremath{\pion^+\pion^-}\xspace}
\def\pipm  {\ensuremath{\pion^\pm}\xspace}
\def\pimp  {\ensuremath{\pion^\mp}\xspace}
\def\pisoft{\ensuremath{\pion_s}\xspace}
\def\kaon  {\ensuremath{\PK}\xspace}
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em \PK}{}\xspace}% do NOT use ensuremath here
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{\kaon^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{\kaon^+}\xspace}
\def\Km    {\ensuremath{\kaon^-}\xspace}
\def\Kpm   {\ensuremath{\kaon^\pm}\xspace}
\def\Kmp   {\ensuremath{\kaon^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{\kaon^0_{\rm\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{\kaon^0_{\rm\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{\kaon^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{\kaon^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{\kaon^{*+}}\xspace}
\def\Kstarm  {\ensuremath{\kaon^{*-}}\xspace}
\def\Kstarpm {\ensuremath{\kaon^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{\kaon^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}

%% Heavy mesons

\def\D       {\ensuremath{\PD}\xspace}
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em \PD}{}\xspace}% do NOT use ensuremath here
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{\D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{\D^+}\xspace}
\def\Dm      {\ensuremath{\D^-}\xspace}
\def\Dpm     {\ensuremath{\D^\pm}\xspace}
\def\Dmp     {\ensuremath{\D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{\D^*}\xspace}
\def\Dsttt   {\ensuremath{\Dstar(2010)^+}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{\D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{\D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{\D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{\D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{\D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{\D^+_\squark}\xspace}
\def\Dsp     {\ensuremath{\D^+_\squark}\xspace}
\def\Dsm     {\ensuremath{\D^-_\squark}\xspace}
\def\Dspm    {\ensuremath{\D^{\pm}_\squark}\xspace}
\def\Dsmp    {\ensuremath{\D^{\mp}_\squark}\xspace}
\def\Dss     {\ensuremath{\D^{*+}_\squark}\xspace}
\def\Dssp    {\ensuremath{\D^{*+}_\squark}\xspace}
\def\Dssm    {\ensuremath{\D^{*-}_\squark}\xspace}
\def\Dsspm   {\ensuremath{\D^{*\pm}_\squark}\xspace}
\def\Dssmp   {\ensuremath{\D^{*\mp}_\squark}\xspace}

\def\B       {\ensuremath{\PB}\xspace}
\def\Bbar    {\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}\xspace}% do NOT use ensuremath here
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BBbar   {\ensuremath{\B\Bbar}\xspace} 
\def\Bz      {\ensuremath{\B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\Bu      {\ensuremath{\B^+}\xspace}
\def\Bub     {\ensuremath{\B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{\B^\pm}\xspace}
\def\Bmp     {\ensuremath{\B^\mp}\xspace}
\def\Bd      {\ensuremath{\B^0}\xspace}
\def\Bs      {\ensuremath{\B^0_\squark}\xspace}
\def\Bsb     {\ensuremath{\Bbar^0_\squark}\xspace}
\def\Bdb     {\ensuremath{\Bbar^0}\xspace}
\def\Bc      {\ensuremath{\B_\cquark^+}\xspace}
\def\Bcp     {\ensuremath{\B_\cquark^+}\xspace}
\def\Bcm     {\ensuremath{\B_\cquark^-}\xspace}
\def\Bcpm    {\ensuremath{\B_\cquark^\pm}\xspace}

%% Onia

\def\jpsi     {\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\Ppsi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\Ppsi(3770)}\xspace}
\def\etac     {\ensuremath{\Peta_\cquark}\xspace}
\def\chiczero {\ensuremath{\Pchi_{\cquark 0}}\xspace}
\def\chicone  {\ensuremath{\Pchi_{\cquark 1}}\xspace}
\def\chictwo  {\ensuremath{\Pchi_{\cquark 2}}\xspace}
\def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

\def\chic  {\ensuremath{\Pchi_{c}}\xspace}

%% Baryons

\def\proton      {\ensuremath{\Pp}\xspace}
\def\antiproton  {\ensuremath{\overline \proton}\xspace}
\def\neutron     {\ensuremath{\Pn}\xspace}
\def\antineutron {\ensuremath{\overline \neutron}\xspace}

\def\Deltares {\ensuremath{\PDelta}\xspace}
\def\Deltaresbar{\ensuremath{\overline \Deltares}\xspace}
\def\Xires {\ensuremath{\PXi}\xspace}
\def\Xiresbar{\ensuremath{\overline \Xires}\xspace}
\def\L {\ensuremath{\PLambda}\xspace}
\def\Lbar {\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}\xspace}
\def\Lambdares {\ensuremath{\PLambda}\xspace}
\def\Lambdaresbar{\ensuremath{\Lbar}\xspace}
\def\Sigmares {\ensuremath{\PSigma}\xspace}
\def\Sigmaresbar{\ensuremath{\overline \Sigmares}\xspace}
\def\Omegares {\ensuremath{\POmega}\xspace}
\def\Omegaresbar{\ensuremath{\overline \Omegares}\xspace}

\def\Lz      {\ensuremath{\L^0}\xspace}
\def\Lzbar   {\ensuremath{\Lbar^0}\xspace}
\def\Lc      {\ensuremath{\L^+_\cquark}\xspace}
\def\Lcbar   {\ensuremath{\Lbar^-_\cquark}\xspace}
\def\Lb      {\ensuremath{\L^0_\bquark}\xspace}
\def\Lbbar   {\ensuremath{\Lbar^0_\bquark}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\cal B}\xspace}}
\def\BRvis      {{\ensuremath{\BR_{\rm{vis}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% EW theory, groups
\def\grpsuthree {\ensuremath{\mathrm{SU}(3)}\xspace}
\def\grpsutw    {\ensuremath{\mathrm{SU}(2)}\xspace}
\def\grpuone    {\ensuremath{\mathrm{U}(1)}\xspace}

\def\ssqtw {\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}\xspace}
\def\csqtw {\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}\xspace}
\def\stw   {\ensuremath{\sin\theta_{\mathrm{W}}}\xspace}
\def\ctw   {\ensuremath{\cos\theta_{\mathrm{W}}}\xspace}
\def\ssqtwef {\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\csqtwef {\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\stwef {\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\ctwef {\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\gv    {\ensuremath{g_{\mbox{\tiny V}}}\xspace}
\def\ga    {\ensuremath{g_{\mbox{\tiny A}}}\xspace}

\def\order   {\ensuremath{\mathcal{O}}\xspace}
\def\ordalph {\ensuremath{\mathcal{O}(\alpha)}\xspace}
\def\ordalsq {\ensuremath{\mathcal{O}(\alpha^{2})}\xspace}
\def\ordalcb {\ensuremath{\mathcal{O}(\alpha^{3})}\xspace}

%% QCD parameters
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}
\def\qsq       {\ensuremath{q^2}\xspace}

%% CKM, CP violation

\def\eps   {\ensuremath{\varepsilon}\xspace}
\def\epsK  {\ensuremath{\varepsilon_K}\xspace}
\def\epsB  {\ensuremath{\varepsilon_B}\xspace}
\def\epsp  {\ensuremath{\varepsilon^\prime_K}\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}

\def\Vud  {\ensuremath{|V_{\uquark\dquark}|}\xspace}
\def\Vcd  {\ensuremath{|V_{\cquark\dquark}|}\xspace}
\def\Vtd  {\ensuremath{|V_{\tquark\dquark}|}\xspace}
\def\Vus  {\ensuremath{|V_{\uquark\squark}|}\xspace}
\def\Vcs  {\ensuremath{|V_{\cquark\squark}|}\xspace}
\def\Vts  {\ensuremath{|V_{\tquark\squark}|}\xspace}
\def\Vub  {\ensuremath{|V_{\uquark\bquark}|}\xspace}
\def\Vcb  {\ensuremath{|V_{\cquark\bquark}|}\xspace}
\def\Vtb  {\ensuremath{|V_{\tquark\bquark}|}\xspace}

%% Oscillations

\newcommand{\dm}{\ensuremath{\Delta m}\xspace}
\newcommand{\dms}{\ensuremath{\Delta m_{\squark}}\xspace}
\newcommand{\dmd}{\ensuremath{\Delta m_{\dquark}}\xspace}
\newcommand{\DG}{\ensuremath{\Delta\Gamma}\xspace}
\newcommand{\DGs}{\ensuremath{\Delta\Gamma_{\squark}}\xspace}
\newcommand{\DGd}{\ensuremath{\Delta\Gamma_{\dquark}}\xspace}
\newcommand{\Gs}{\ensuremath{\Gamma_{\squark}}\xspace}
\newcommand{\Gd}{\ensuremath{\Gamma_{\dquark}}\xspace}

\newcommand{\MBq}{\ensuremath{M_{\B_\quark}}\xspace}
\newcommand{\DGq}{\ensuremath{\Delta\Gamma_{\quark}}\xspace}
\newcommand{\Gq}{\ensuremath{\Gamma_{\quark}}\xspace}
\newcommand{\dmq}{\ensuremath{\Delta m_{\quark}}\xspace}
\newcommand{\GL}{\ensuremath{\Gamma_{\rm L}}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_{\rm H}}\xspace}

\newcommand{\ACP}{\ensuremath{{\cal A}^{\CP}}\xspace}
\newcommand{\Adir}{\ensuremath{{\cal A}^{\rm dir}}\xspace}
\newcommand{\Amix}{\ensuremath{{\cal A}^{\rm mix}}\xspace}
\newcommand{\ADelta}{\ensuremath{{\cal A}^\Delta}\xspace}

%% Tagging
\newcommand{\eff}{{\ensuremath{\varepsilon}}\xspace}
\newcommand{\efftag}{{\ensuremath{\varepsilon_{\rm tag}}}\xspace}
\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\effeff}{{\ensuremath{\varepsilon_{\rm eff}}}\xspace}
\newcommand{\efftageff}{{\ensuremath{\varepsilon^{\rm eff}_{\rm tag}}}\xspace}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\rm\,#1}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\rm m}\xspace}
\def\muma {\ensuremath{\,\upmu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mub{\ensuremath{\rm \,\upmu b}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\nb {\ensuremath{\rm \,nb}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\rm {\,s}}\xspace}
\def\ms   {\ensuremath{{\rm \,ms}}\xspace}
\def\mus  {\ensuremath{\,\upmu{\rm s}}\xspace}
\def\ns   {\ensuremath{{\rm \,ns}}\xspace}
\def\ps   {\ensuremath{{\rm \,ps}}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}

\def\mhz  {\ensuremath{{\rm \,MHz}}\xspace}
\def\khz  {\ensuremath{{\rm \,kHz}}\xspace}
\def\hz   {\ensuremath{{\rm \,Hz}}\xspace}

\def\invps{\ensuremath{{\rm \,ps^{-1}}}\xspace}

\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}

%% Angles
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}
\def\rad{\ensuremath{\rm \,rad}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\rm \,n_{eq}}\xspace}
\def\neqcmcm {\ensuremath{\rm \,n_{eq} / cm^2}\xspace}
\def\kRad {\ensuremath{\rm \,kRad}\xspace}
\def\MRad {\ensuremath{\rm \,MRad}\xspace}
\def\ci {\ensuremath{\rm \,Ci}\xspace}
\def\mci {\ensuremath{\rm \,mCi}\xspace}

%% Uncertainties
\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

%% Maths
\def\order{{\ensuremath{\cal O}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chisq/\mathrm{ndf}}\xspace}
\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\sPlot{\mbox{\em sPlot}}
\def\sWeight{\mbox{\em sWeight}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\pt         {\mbox{$p_{\rm T}$}\xspace}
\def\et         {\mbox{$E_{\rm T}$}\xspace}

\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
\def\evtgen   {\mbox{\textsc{EvtGen}}\xspace}
\def\pythia    {\mbox{\textsc{Pythia8}}\xspace}
\def\kkmc     {\mbox{\textsc{KKMC}}\xspace}
\def\geant     {\mbox{\textsc{Geant4}}\xspace}
\def\photos   {\mbox{\textsc{Photos}}\xspace}
\def\tauola    {\mbox{\textsc{TAUOLA}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\pyroot   {\mbox{\textsc{PyRoot}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}}
\newcommand{\etal}{{\slshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}


==> material.tex <==
% INCLUDE ALL FIGURES AND NUMBERS THAT SHOULD BE APPROVED FOR PUBLIC PRESENTATION IN THIS FILE.
 \section*{Additional Material}
% This sections contains all figures and numbers that are requested to be approved for public presentation.
To prevent excluding a phase space region that may affect various New Physics model candidates for \tautomumumu LFV decays, we provide the Dalitz plots shown in Figure~\ref{fig: Dalitz plots}. 
\begin{figure}[H]
    \centering
  
    \includegraphics[page=18,width=0.8\columnwidth]{figures/Plot_DataMC_Sideband_TotalNetChargeZero_dmID333_thrust_LID095_BDT090.pdf}
    \caption{Signal distribution in the 2D plane defined by the mass squared of the opposite charge muons, for candidates passing the full selection.}
    \label{fig: Dalitz plots}
\end{figure}

==> pacs.tex <==
% WRITE THE PACS CODES IN THIS FILE.


==> pub074.tex <==
%%% Paper:    tau to ell KS
%%% Journal:  JHEP
%%% Contacts: K. Lautenbach, L. Zani, J. Serrano
%%% ====================================================================
%%% Use \input{pub074} to insert this material into your latex file.
\newcounter{AffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCPPM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYerevan{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instGoettingen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBeihang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBINP{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instCMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCinvestavIPN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPrague{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChiangMai{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instChiba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChonnam{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instChula{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCAU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instConacyt{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDESY{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instDuke{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instITAR{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFuJen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFudan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGifu{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSOKENDAI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMainz{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGyeongsang{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHanyang{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHeidelberg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKEK{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJPARC{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instHiroshima{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHUNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFrascati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteINFN{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIISc{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instIISER{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITBhubaneswar{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITGuwahati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITHyderabad{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITJodhpur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIITMadras{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIndiana{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPRussia{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHEPHYVienna{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIHEPChina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIOP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIFIC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instISU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJAEA{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instJLU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKarlsruhe{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKitasato{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKISTI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKoreaUnivKU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyotoU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instKyungpook{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instLNNU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instGiessen{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLuther{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMNITJaipur{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMcGill{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMETU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMEPhI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNagoyaKMI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNankai{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNaraWu{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUNAM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHSE{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNTUTaiwan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKrakow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNiigata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNSU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instOsakaMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRCNP{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPNNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMPP{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMPGHLL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPanjabPAU{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instRIKENBNL{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRIKENMSL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSeoul{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instShandong{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instKyiv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSPU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoochow{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSoongsil{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSEU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaJSI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSKKU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTelAviv{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instToho{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTohoku{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTitech{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instTokyoMetropolitan{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUAS{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instNapoliUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPadovaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPerugiaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPisaUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instRomaTreUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTorinoUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTriesteUNIV{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIJCLab{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPHC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instAdelaide{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUofA{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instBonn{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUBC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instCincinnati{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instFlorida{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHamburg{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instHawaii{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUniLJ{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLouisville{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instMalaya{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instManitoba{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instLjubljanaUM{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMelbourne{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instMississippi{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instUOM{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instNovaGorica{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUPES{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instPittsburgh{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUSTC{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSAlabama{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instSCarolina{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instSydney{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTabuk{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUTokyo{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instEri{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instIPMU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVictoria{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instUppsala{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instVPI{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instWayneState{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instXavier{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instXJTU{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYamagata{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instYonsei{\protect\theAffiliationCounter}
\stepcounter{AffiliationCounter}\edef\instTYL{\protect\theAffiliationCounter}
%%%\stepcounter{AffiliationCounter}\edef\instZZU{\protect\theAffiliationCounter}
\collaboration{The Belle and Belle II Collaborations}
  \author[\instKEK,\instSOKENDAI]{I.~Adachi,} % 2590
% \author[\instKrakow]{K.~Adamczyk,} % 2239
  \author[\instPanjab]{L.~Aggarwal,} % 10083
% \author[\instBonn]{P.~Ahlburg,} % 2367
  \author[\instXavier]{H.~Ahmed,} % 11323
% \author[\instKoreaUnivKU]{J.~K.~Ahn,} % 7423
  \author[\instKoreaUnivKU]{Y.~Ahn,} % 14363
  \author[\instUTokyo]{H.~Aihara,} % 2223
  \author[\instYerevan]{N.~Akopov,} % 9443
  \author[\instTabuk]{S.~Alghamdi,} % 27804
  \author[\instTabuk]{M.~Alhakami,} % 28103
  \author[\instNapoliUNIV,\instNapoliINFN]{A.~Aloisio,} % 2194
% \author[\instTabuk]{S.~Al~Said,} % 6823
  \author[\instTabuk]{N.~Althubiti,} % 21524
  \author[\instTriesteUNIV,\instTriesteINFN]{K.~Amos,} % 27583
% \author[\instMPGHLL]{L.~Andricek,} % 2098
  \author[\instBonn]{M.~Angelsmark,} % 13963
  \author[\instIOP]{N.~Anh~Ky,} % 2218
  \author[\instPadovaUNIV,\instPadovaINFN]{C.~Antonioli,} % 20583
  \author[\instHawaii]{D.~M.~Asner,} % 4684
  \author[\instCincinnati]{H.~Atmacan,} % 2538
% \author[\instBINP,\instNSU]{V.~Aulchenko,} % 8183
% \author[\instHSE]{T.~Aushev,} % 3747
  \author[\instKyiv]{V.~Aushev,} % 2155
  \author[\instNagoya]{M.~Aversano,} % 7363
  \author[\instTabuk]{R.~Ayad,} % 3766
% \author[\instTata]{T.~Aziz,} % 3523
  \author[\instIPHC]{V.~Babu,} % 5623
% \author[\instKrakow]{S.~Bacher,} % 2258
% \author[\instKEK]{H.~Bae,} % 10863
  \author[\instLouisville]{N.~K.~Baghel,} % 21505
  \author[\instIITBhubaneswar]{S.~Bahinipati,} % 2332
% \author[\instSydney]{A.~M.~Bakich,} % 2115
  \author[\instIJCLab]{P.~Bambade,} % 3003
  \author[\instLouisville]{Sw.~Banerjee,} % 8603
% \author[\instPanjab]{S.~Bansal,} % 5163
  \author[\instKEK]{M.~Barrett,} % 2180
  \author[\instMPP]{M.~Bartl,} % 26483
% \author[\instPisaUNIV,\instPisaINFN]{G.~Batignani,} % 6643
  \author[\instIPHC]{J.~Baudot,} % 2562
% \author[\instKarlsruhe]{M.~Bauer,} % 9863
  \author[\instDESY]{A.~Baur,} % 5683
  \author[\instVictoria]{A.~Beaubien,} % 6683
  \author[\instDESY]{F.~Becherer,} % 21623
  \author[\instKarlsruhe]{J.~Becker,} % 5403
% \author[\instIITMadras]{P.~K.~Behera,} % 4204
% \author[\instIHEPRussia]{K.~Belous,} % 2329
  \author[\instMississippi]{J.~V.~Bennett,} % 2454
% \author[\instRomaTreINFN]{E.~Bernieri,} % 4483
  \author[\instBonn]{F.~U.~Bernlochner,} % 2282
  \author[\instBonn]{V.~Bertacchi,} % 2212
  \author[\instHEPHYVienna]{M.~Bertemes,} % 2595
  \author[\instTelAviv]{E.~Bertholet,} % 13163
  \author[\instHawaii]{M.~Bessner,} % 3783
% \author[\instMEPhI]{D.~Z.~Besson,} % 3585
  \author[\instPisaUNIV,\instPisaINFN]{S.~Bettarini,} % 2350
% \author[\instIISER]{V.~Bhardwaj,} % 2228
  \author[\instIITGuwahati]{B.~Bhuyan,} % 2097
  \author[\instTorinoUNIV,\instTorinoINFN]{F.~Bianchi,} % 2564
% \author[\instTUM]{L.~Bierwirth,} % 11723
% \author[\instDESY]{T.~Bilka,} % 2484
% \author[\instLMU]{S.~Bilokin,} % 3623
  \author[\instLouisville]{D.~Biswas,} % 8703
% \author[\instKEK]{T.~Bloomfield,} % 2418
  \author[\instBINP,\instNSU]{A.~Bobrov,} % 2294
  \author[\instSoochow,\instHSE]{D.~Bodrov,} % 9643
% \author[\instDESY]{A.~Bolz,} % 15403
  \author[\instBINP,\instNSU]{A.~Bondar,} % 4643
  \author[\instWayneState]{G.~Bonvicini,} % 2095
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{J.~Borah,} % 7083
  \author[\instTorinoUNIV,\instTorinoINFN]{A.~Boschetti,} % 17683
  \author[\instKrakow]{A.~Bozek,} % 2303
  \author[\instLjubljanaJSI,\instLjubljanaUM]{M.~Bra\v{c}ko,} % 2425
  \author[\instRomaTreINFN]{P.~Branchini,} % 2577
% \author[\instISU]{N.~Brenny,} % 19943
% \author[\instCMU]{R.~A.~Briere,} % 2584
  \author[\instHawaii]{T.~E.~Browder,} % 2560
% \author[\instGoettingen]{Y.~Buch,} % 17323
  \author[\instRomaTreINFN]{A.~Budano,} % 2171
  \author[\instRomaTreUNIV,\instRomaTreINFN]{S.~Bussino,} % 5384
% \author[\instFrascati]{A.~Calcaterra,} % 19163
% \author[\instMPP]{A.~Caldwell,} % 2608
  \author[\instMississippi]{Q.~Campagna,} % 21563
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Campajola,} % 5223
  \author[\instDESY]{L.~Cao,} % 2099
  \author[\instPisaUNIV,\instPisaINFN]{G.~Casarosa,} % 2491
  \author[\instPerugiaUNIV,\instPerugiaINFN]{C.~Cecchi,} % 2433
% \author[\instIPHC]{J.~Cerasoli,} % 20746
  \author[\instFuJen]{M.-C.~Chang,} % 2827
% \author[\instNTUTaiwan]{P.~Chang,} % 2542
  \author[\instDESY]{R.~Cheaib,} % 2208
  \author[\instSydney]{P.~Cheema,} % 15264
% \author[\instMPP]{V.~Chekelian,} % 2167
% \author[\instISU]{C.~Chen,} % 12803
% \author[\instJLU]{Y.~Q.~Chen,} % 16264
% \author[\instNTUTaiwan]{Y.-T.~Chen,} % 2884
  \author[\instHanyang]{B.~G.~Cheon,} % 2173
  \author[\instBINP]{K.~Chilikin,} % 2308
  \author[\instCincinnati]{J.~Chin,} % 20283
  \author[\instChiangMai]{K.~Chirapatpimol,} % 10803
  \author[\instHanyang]{H.-E.~Cho,} % 2182
  \author[\instKISTI]{K.~Cho,} % 2516
  \author[\instYonsei]{S.-J.~Cho,} % 2723
  \author[\instCAU]{S.-K.~Choi,} % 2364
  \author[\instISU]{S.~Choudhury,} % 2206
% \author[\instMcGill]{K.~Chu,} % 5203
% \author[\instWayneState]{D.~Cinabro,} % 2092
  \author[\instISU]{J.~Cochran,} % 12604
  \author[\instCPPM]{I.~Consigny,} % 23903
  \author[\instPisaUNIV,\instPisaINFN]{L.~Corona,} % 3944
% \author[\instMississippi]{L.~M.~Cremaldi,} % 2276
  \author[\instSEU]{J.~X.~Cui,} % 8863
% \author[\instTokyoMetropolitan]{T.~Czank,} % 2254
% \author[\instMNITJaipur]{S.~Das,} % 9163
% \author[\instDESY]{F.~Dattola,} % 3745
  \author[\instCinvestavIPN]{E.~De~La~Cruz-Burelo,} % 2359
  \author[\instAdelaide,\instTorinoUNIV,\instTorinoINFN]{S.~A.~De~La~Motte,} % 2128
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{G.~de~Marino,} % 8364
  \author[\instNapoliUNIV,\instNapoliINFN]{G.~De~Nardo,} % 2459
% \author[\instUBC]{M.~De~Nuccio,} % 2610
  \author[\instKarlsruhe]{G.~De~Pietro,} % 2528
  \author[\instFrascati]{R.~de~Sangro,} % 2524
% \author[\instBonn]{B.~Deschamps,} % 2671
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Destefanis,} % 2594
  \author[\instKEK]{S.~Dey,} % 5023
% \author[\instCinvestavIPN]{A.~De~Yta-Hernandez,} % 2104
% \author[\instIITHyderabad]{R.~Dhamija,} % 9465
  \author[\instBNL]{A.~Di~Canto,} % 10963
% \author[\instNapoliUNIV,\instNapoliINFN]{F.~Di~Capua,} % 2065
  \author[\instBonn]{J.~Dingfelder,} % 2151
  \author[\instPrague]{Z.~Dole\v{z}al,} % 2319
  \author[\instUAS]{I.~Dom\'{\i}nguez~Jim\'{e}nez,} % 2191
  \author[\instITAR]{T.~V.~Dong,} % 2215
% \author[\instDESY]{X.~Dong,} % 17343
  \author[\instTriesteINFN]{M.~Dorigo,} % 12543
% \author[\instHEPHYVienna]{D.~Dorner,} % 13564
% \author[\instGiessen]{K.~Dort,} % 5583
% \author[\instMelbourne]{D.~Dossett,} % 2574
% \author[\instDESY]{S.~Dreyer,} % 12823
% \author[\instHawaii]{S.~Dubey,} % 11063
% \author[\instBonn]{S.~Duell,} % 2344
  \author[\instTUM]{K.~Dugic,} % 11103
  \author[\instIPHC]{G.~Dujany,} % 9703
  \author[\instKarlsruhe]{P.~Ecker,} % 5563
% \author[\instBonn]{M.~Eliachevitch,} % 2725
  \author[\instBINP,\instNSU]{D.~Epifanov,} % 2551
  \author[\instKarlsruhe]{J.~Eppelt,} % 19723
% \author[\instDESY]{Y.~Fan,} % 21303
% \author[\instBonn]{R.~Farkas,} % 12843
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{P.~Feichtinger,} % 9843
  \author[\instKarlsruhe]{T.~Ferber,} % 2482
% \author[\instMelbourne]{D.~Ferlewicz,} % 2073
  \author[\instKEK]{T.~Fillinger,} % 9803
  \author[\instIPHC]{C.~Finck,} % 15803
  \author[\instFrascati]{G.~Finocchiaro,} % 2400
% \author[\instHeidelberg]{P.~Fischer,} % 2141
% \author[\instHawaii]{K.~Flood,} % 12103
  \author[\instMcGill]{A.~Fodor,} % 2312
  \author[\instPisaUNIV,\instPisaINFN]{F.~Forti,} % 2432
% \author[\instGoettingen]{A.~Frey,} % 2150
% \author[\instHEPHYVienna]{M.~Friedl,} % 2442
  \author[\instPNNL]{B.~G.~Fulsom,} % 2563
  \author[\instPisaINFN]{A.~Gabrielli,} % 13523
% \author[\instBINP,\instNSU]{N.~Gabyshev,} % 2510
  \author[\instCincinnati]{A.~Gale,} % 20263
% \author[\instDESY]{E.~Ganiev,} % 4623
  \author[\instKEK]{M.~Garcia-Hernandez,} % 4823
% \author[\instCMU]{R.~Garg,} % 2213
% \author[\instBINP,\instNSU]{A.~Garmash,} % 2161
% \author[\instLMU]{L.~G\"artner,} % 21783
  \author[\instNapoliINFN]{G.~Gaudino,} % 16563
  \author[\instUPES]{V.~Gaur,} % 2413
  \author[\instIITBhubaneswar]{V.~Gautam,} % 22223
  \author[\instPadovaUNIV,\instPadovaINFN]{A.~Gaz,} % 2181
% \author[\instGoettingen]{U.~Gebauer,} % 2174
  \author[\instDESY]{A.~Gellrich,} % 2480
  \author[\instYerevan]{G.~Ghevondyan,} % 9445
  \author[\instTriesteUNIV,\instTriesteINFN]{D.~Ghosh,} % 11923
  \author[\instYerevan]{H.~Ghumaryan,} % 19543
  \author[\instBonn]{G.~Giakoustidis,} % 13723
  \author[\instNapoliUNIV,\instNapoliINFN]{R.~Giordano,} % 2103
  \author[\instIITHyderabad]{A.~Giri,} % 2106
  \author[\instIPHC]{P.~Gironella~Gironell,} % 25443
  \author[\instDESY]{A.~Glazov,} % 2473
  \author[\instTriesteINFN]{B.~Gobbo,} % 2109
  \author[\instSAlabama]{R.~Godang,} % 2449
% \author[\instKyiv]{O.~Gogota,} % 2334
  \author[\instKarlsruhe]{P.~Goldenzweig,} % 2345
% \author[\instNovaGorica,\instLjubljanaJSI]{B.~Golob,} % 3703
% \author[\instUSTC]{G.~Gong,} % 2727
% \author[\instAdelaide]{P.~Grace,} % 9563
  \author[\instMainz]{W.~Gradl,} % 2570
% \author[\instDESY]{M.~Graf-Schreiber,} % 2730
% \author[\instVictoria]{T.~Grammatico,} % 20623
% \author[\instBonn]{S.~Granderath,} % 8383
  \author[\instRomaTreINFN]{E.~Graziani,} % 2342
  \author[\instTUM]{D.~Greenwald,} % 2686
  \author[\instPrague]{Z.~Gruberov\'{a},} % 8824
% \author[\instPittsburgh]{T.~Gu,} % 14283
  \author[\instCincinnati]{Y.~Guan,} % 2514
  \author[\instBINP,\instNSU]{K.~Gudkova,} % 10504
  \author[\instKarlsruhe]{I.~Haide,} % 14824
% \author[\instHEPHYVienna]{H.~Haigh,} % 16744
% \author[\instTata]{S.~Halder,} % 4743
  \author[\instDESY]{Y.~Han,} % 19663
% \author[\instKEK,\instSOKENDAI]{K.~Hara,} % 2462
  \author[\instKEK,\instSOKENDAI]{T.~Hara,} % 2523
% \author[\instAdelaide]{C.~Harris,} % 21383
% \author[\instHawaii]{O.~Hartbrich,} % 2158
  \author[\instNiigata]{K.~Hayasaka,} % 2330
  \author[\instNaraWu]{H.~Hayashii,} % 2455
  \author[\instMPP]{S.~Hazra,} % 7663
  \author[\instUBC,\instIPP]{C.~Hearty,} % 2450
  \author[\instBonn]{M.~T.~Hedges,} % 2265
  \author[\instKarlsruhe]{A.~Heidelbach,} % 16923
  \author[\instCinvestavIPN,\instConacyt]{I.~Heredia~de~la~Cruz,} % 2559
  \author[\instBNL]{M.~Hern\'{a}ndez~Villanueva,} % 2466
  \author[\instIPMU]{T.~Higuchi,} % 2485
% \author[\instNagoya]{H.~Hirata,} % 2070
  \author[\instMainz]{M.~Hoek,} % 2101
  \author[\instMelbourne]{M.~Hohmann,} % 2077
  \author[\instDESY]{R.~Hoppe,} % 23383
  \author[\instHEPHYVienna]{P.~Horak,} % 13583
% \author[\instRCNP]{T.~Hotta,} % 2084
  \author[\instSydney]{C.-L.~Hsu,} % 2299
% \author[\instSydney]{A.~Huang,} % 14223
% \author[\instNTUTaiwan]{K.~Huang,} % 2389
  \author[\instDESY]{T.~Humair,} % 10643
  \author[\instNagoya,\instNagoyaKMI,\instKEK]{T.~Iijima,} % 2446
  \author[\instNagoya,\instKEK]{K.~Inami,} % 2323
  \author[\instHEPHYVienna]{G.~Inguglia,} % 2500
  \author[\instIITHyderabad]{N.~Ipsita,} % 12223
% \author[\instHEPHYVienna]{C.~Irmler,} % 2186
  \author[\instKEK,\instSOKENDAI]{A.~Ishikawa,} % 2281
% \author[\instKEK]{S.~Ito,} % 17463
  \author[\instKEK,\instSOKENDAI]{R.~Itoh,} % 2487
  \author[\instOsakaMetropolitan]{M.~Iwasaki,} % 2360
% \author[\instKEK]{Y.~Iwasaki,} % 2229
% \author[\instTokyoMetropolitan]{S.~Iwata,} % 4323
  \author[\instAdelaide]{P.~Jackson,} % 2255
  \author[\instBonn]{D.~Jacobi,} % 15123
  \author[\instIndiana]{W.~W.~Jacobs,} % 2322
  \author[\instBNL]{D.~E.~Jaffe,} % 3663
  \author[\instGyeongsang]{E.-J.~Jang,} % 6744
% \author[\instHNU]{Q.~P.~Ji,} % 16243
% \author[\instIHEPChina]{X.~B.~Ji,} % 2558
  \author[\instSEU]{S.~Jia,} % 2457
  \author[\instBNL]{Y.~Jin,} % 2105
  \author[\instIITMadras]{A.~Johnson,} % 16143
  \author[\instChonnam]{K.~K.~Joo,} % 4224
  \author[\instBonn]{H.~Junkerkalefeld,} % 12963
% \author[\instKyiv]{I.~Kadenko,} % 3843
% \author[\instTokyoMetropolitan]{H.~Kakuno,} % 2391
% \author[\instKrakow]{M.~Kaleta,} % 5603
% \author[\instIITGuwahati]{D.~Kalita,} % 2220
  \author[\instHEPHYVienna]{A.~B.~Kaliyar,} % 7344
  \author[\instPadovaINFN]{J.~Kandra,} % 2541
  \author[\instIPMU]{K.~H.~Kang,} % 2283
% \author[\instISU]{S.~Kang,} % 12683
  \author[\instYerevan]{G.~Karyan,} % 2550
% \author[\instChiba]{H.~Kawai,} % 4344
  \author[\instKitasato]{T.~Kawasaki,} % 4363
  \author[\instMainz]{F.~Keil,} % 19523
  \author[\instHawaii]{C.~Ketter,} % 2236
% \author[\instBonn]{M.~Khan,} % 15644
  \author[\instMPP]{C.~Kiesling,} % 2168
% \author[\instYonsei]{C.~Kim,} % 20503
  \author[\instHanyang]{C.-H.~Kim,} % 2358
  \author[\instSoongsil]{D.~Y.~Kim,} % 2315
  \author[\instYonsei]{J.-Y.~Kim,} % 20223
  \author[\instKISTI]{K.-H.~Kim,} % 2118
% \author[\instSeoul]{S.~K.~Kim,} % 3823
  \author[\instKoreaUnivKU]{Y.~J.~Kim,} % 2403
% \author[\instYonsei]{Y.-K.~Kim,} % 2379
  \author[\instVPI,\instKEK]{H.~Kindo,} % 2195
  \author[\instCincinnati]{K.~Kinoshita,} % 2318
% \author[\instDESY]{C.~Kleinwort,} % 2499
  \author[\instPrague]{P.~Kody\v{s},} % 2407
  \author[\instKEK]{T.~Koga,} % 6963
  \author[\instHawaii]{S.~Kohani,} % 9143
  \author[\instNagoya]{K.~Kojima,} % 6363
% \author[\instKitasato]{T.~Konno,} % 2490
% \author[\instHawaii]{H.~Korandla,} % 18783
  \author[\instBINP,\instNSU]{A.~Korobov,} % 4185
  \author[\instLjubljanaJSI,\instLjubljanaUM]{S.~Korpar,} % 2475
% \author[\instIJCLab]{E.~Kou,} % 3765
  \author[\instBINP,\instNSU]{E.~Kovalenko,} % 3884
  \author[\instVictoria]{R.~Kowalewski,} % 2293
% \author[\instMPP]{T.~M.~G.~Kraetzschmar,} % 7543
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{P.~Kri\v{z}an,} % 2474
% \author[\instMississippi]{R.~Kroeger,} % 2242
  \author[\instBINP,\instNSU]{P.~Krokovny,} % 2575
% \author[\instGiessen]{W.~Kuehn,} % 2534
  \author[\instLMU]{T.~Kuhr,} % 2486
  \author[\instLMU]{Y.~Kulii,} % 9823
  \author[\instIITGuwahati]{D.~Kumar,} % 7223
  \author[\instIITJodhpur]{J.~Kumar,} % 6464
% \author[\instIISER]{M.~Kumar,} % 2744
  \author[\instPanjabPAU]{R.~Kumar,} % 2189
  \author[\instMississippi]{K.~Kumara,} % 2257
% \author[\instTokyoMetropolitan]{T.~Kumita,} % 4083
  \author[\instKEK]{T.~Kunigo,} % 10104
% \author[\instNaraWu]{A.~Kusudo,} % 14623
  \author[\instBINP,\instNSU]{A.~Kuzmin,} % 2520
% \author[\instPrague]{P.~Kvasni\v{c}ka,} % 2184
  \author[\instYonsei]{Y.-J.~Kwon,} % 2231
  \author[\instPadovaINFN]{S.~Lacaprara,} % 2447
% \author[\instKEK]{Y.-T.~Lai,} % 2066
  \author[\instMNITJaipur]{K.~Lalwani,} % 2142
  \author[\instVPI]{T.~Lam,} % 2729
  \author[\instTriesteINFN]{L.~Lanceri,} % 2540
  \author[\instGiessen]{J.~S.~Lange,} % 2277
  \author[\instKEK]{T.~S.~Lau,} % 19803
  \author[\instUppsala]{M.~Laurenza,} % 10223
% \author[\instCPPM]{K.~Lautenbach,} % 2102
% \author[\instBNL]{P.~J.~Laycock,} % 7683
  \author[\instUBC]{R.~Leboucher,} % 14083
  \author[\instIJCLab]{F.~R.~Le~Diberder,} % 3267
% \author[\instSeoul]{J.~Lee,} % 2190
  \author[\instSKKU]{M.~J.~Lee,} % 21803
% \author[\instMPP]{P.~Leitl,} % 2414
  \author[\instCPPM]{C.~Lemettais,} % 22704
  \author[\instDESY,\instHamburg]{P.~Leo,} % 19823
% \author[\instKEK]{D.~Levit,} % 2507
% \author[\instHawaii]{P.~M.~Lewis,} % 2582
% \author[\instLNNU]{C.~Li,} % 2325
  \author[\instHNU]{H.-J.~Li,} % 4943
  \author[\instCincinnati]{L.~K.~Li,} % 3263
  \author[\instIHEPChina]{Q.~M.~Li,} % 22943
% \author[\instFudan]{S.~X.~Li,} % 2377
  \author[\instBeihang]{W.~Z.~Li,} % 19703
  \author[\instFudan]{Y.~Li,} % 8083
  \author[\instXJTU]{Y.~B.~Li,} % 2573
  \author[\instIHEPChina]{Y.~P.~Liao,} % 24303
  \author[\instIITMadras]{J.~Libby,} % 2262
  \author[\instNTUTaiwan]{J.~Lin,} % 2401
  \author[\instPadovaUNIV,\instPadovaINFN]{S.~Lin,} % 17223
% \author[\instHiroshima]{Z.~Liptak,} % 3565
  \author[\instCPPM]{V.~Lisovskyi,} % 26584
% \author[\instSydney]{A.~Little,} % 23803
  \author[\instJLU]{M.~H.~Liu,} % 15244
  \author[\instHawaii]{Q.~Y.~Liu,} % 7045
  \author[\instKEK,\instSOKENDAI]{Y.~Liu,} % 16223
% \author[\instIHEPChina]{Z.~A.~Liu,} % 3283
  \author[\instShandong]{Z.~Q.~Liu,} % 11303
  \author[\instWayneState,\instKEK]{D.~Liventsev,} % 2578
  \author[\instManitoba]{S.~Longo,} % 2396
% \author[\instCinvestavIPN]{G.~Lopez-Castro,} % 4245
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Lozar,} % 12423
  \author[\instLMU]{T.~Lueck,} % 2406
% \author[\instFudan]{T.~Luo,} % 3268
  \author[\instBonn]{C.~Lyu,} % 12484
  \author[\instRIKENMSL]{Y.~Ma,} % 16883
  \author[\instTata]{C.~Madaan,} % 25483
% \author[\instNagoya]{A.~Maeda,} % 14664
  \author[\instTorinoUNIV,\instTorinoINFN]{M.~Maggiora,} % 5343
  \author[\instIITHyderabad]{S.~P.~Maharana,} % 19083
% \author[\instHawaii]{T.~Mahood,} % 26003
  \author[\instTorinoINFN]{R.~Maiti,} % 12043
% \author[\instIITBhubaneswar]{S.~Maity,} % 2985
  \author[\instCPPM]{G.~Mancinelli,} % 20743
  \author[\instBNL]{R.~Manfredi,} % 10303
  \author[\instPerugiaINFN]{E.~Manoni,} % 2305
% \author[\instBonn]{A.~C.~Manthei,} % 15023
  \author[\instTriesteUNIV,\instTriesteINFN]{M.~Mantovano,} % 19783
  \author[\instMelbourne]{D.~Marcantonio,} % 11163
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Marcello,} % 4223
  \author[\instIFIC]{C.~Marinas,} % 2133
  \author[\instRomaTreINFN]{C.~Martellini,} % 16983
  \author[\instIJCLab]{A.~Martens,} % 13823
  \author[\instDESY]{A.~Martini,} % 2336
  \author[\instDESY]{T.~Martinov,} % 19463
  \author[\instPisaUNIV,\instPisaINFN]{L.~Massaccesi,} % 16323
  \author[\instRCNP,\instEri]{M.~Masuda,} % 2238
% \author[\instUOM]{T.~Matsuda,} % 5543
% \author[\instKEK,\instNagoya]{K.~Matsuoka,} % 2316
  \author[\instBINP,\instNSU]{D.~Matvienko,} % 2351
  \author[\instIITGuwahati]{S.~K.~Maurya,} % 9763
  \author[\instIPHC]{M.~Maushart,} % 21203
% \author[\instIJCLab]{F.~Mawas,} % 20943
  \author[\instUBC]{J.~A.~McKenna,} % 2392
% \author[\instMPP]{F.~Meggendorfer,} % 7103
  \author[\instTata]{R.~Mehta,} % 15203
  \author[\instDuke]{F.~Meier,} % 3103
  \author[\instGiessen]{D.~Meleshko,} % 11523
  \author[\instNapoliUNIV,\instNapoliINFN]{M.~Merola,} % 2456
% \author[\instBonn]{F.~Metzner,} % 2296
% \author[\instMelbourne]{M.~Milesi,} % 5443
  \author[\instVictoria]{C.~Miller,} % 2273
  \author[\instNapoliINFN]{M.~Mirra,} % 14744
  \author[\instISU]{S.~Mitra,} % 19944
  \author[\instNaraWu,\instKEK]{K.~Miyabayashi,} % 2327
  \author[\instKEK,\instSOKENDAI]{H.~Miyake,} % 2452
  \author[\instIJCLab]{R.~Mizuk,} % 2483
  \author[\instTata]{G.~B.~Mohanty,} % 2278
% \author[\instCinvestavIPN]{N.~Molina-Gonzalez,} % 8004
  \author[\instPisaUNIV,\instPisaINFN]{S.~Mondal,} % 19743
  \author[\instPerugiaUNIV,\instPerugiaINFN]{S.~Moneta,} % 13303
% \author[\instKoreaUnivKU]{H.~Moon,} % 2304
  \author[\instDESY]{A.~L.~Moreira~de~Carvalho,} % 26403
  \author[\instMPP]{H.-G.~Moser,} % 2120
% \author[\instHEPHYVienna]{M.~Mrvar,} % 2527
% \author[\instKarlsruhe]{Th.~Muller,} % 2165
% \author[\instTorinoINFN]{R.~Mussa,} % 2372
  \author[\instKEK,\instSOKENDAI]{I.~Nakamura,} % 3463
% \author[\instKEK,\instSOKENDAI]{K.~R.~Nakamura,} % 2417
% \author[\instOsakaMetropolitan]{E.~Nakano,} % 2554
% \author[\instRCNP]{T.~Nakano,} % 2983
  \author[\instKEK,\instSOKENDAI]{M.~Nakao,} % 2498
% \author[\instKEK,\instSOKENDAI]{H.~Nakayama,} % 2232
% \author[\instNTUTaiwan]{H.~Nakazawa,} % 2335
  \author[\instKEK]{Y.~Nakazawa,} % 17383
% \author[\instDESY]{A.~Narimani~Charan,} % 10143
  \author[\instKyotoU]{M.~Naruki,} % 4583
  \author[\instKrakow]{Z.~Natkaniec,} % 3923
  \author[\instBNL]{A.~Natochii,} % 12063
% \author[\instIITHyderabad]{L.~Nayak,} % 9464
  \author[\instIISc]{M.~Nayak,} % 2371
% \author[\instYerevan]{G.~Nazaryan,} % 9523
  \author[\instKarlsruhe]{M.~Neu,} % 23304
% \author[\instDESY]{C.~Niebuhr,} % 2477
% \author[\instKSU]{M.~Niiyama,} % 2063
% \author[\instMPGHLL]{J.~Ninkovic,} % 2386
% \author[\instBNL]{N.~K.~Nisar,} % 2522
  \author[\instKEK,\instSOKENDAI,\instNiigata]{S.~Nishida,} % 2571
% \author[\instHawaii]{K.~Nishimura,} % 3063
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{A.~Novosel,} % 15523
  \author[\instToho]{S.~Ogawa,} % 6263
  \author[\instNagoya]{R.~Okubo,} % 10743
% \author[\instCAU]{S.~L.~Olsen,} % 4563
% \author[\instKyiv]{Y.~Onishchuk,} % 2157
  \author[\instNiigata]{H.~Ono,} % 2160
  \author[\instUTokyo]{Y.~Onuki,} % 2331
% \author[\instIJCLab]{P.~Oskin,} % 9623
% \author[\instUTokyo]{F.~Otani,} % 16244
% \author[\instCMU]{E.~R.~Oxford,} % 6943
% \author[\instKEK,\instSOKENDAI]{H.~Ozaki,} % 2984
% \author[\instHSE]{P.~Pakhlov,} % 2221
  \author[\instHSE]{G.~Pakhlova,} % 2188
% \author[\instPisaUNIV,\instPisaINFN]{A.~Paladino,} % 2435
% \author[\instMississippi]{A.~Panta,} % 7943
% \author[\instPisaUNIV,\instPisaINFN]{E.~Paoloni,} % 2488
  \author[\instNapoliINFN]{S.~Pardi,} % 2532
  \author[\instDuke]{K.~Parham,} % 10684
% \author[\instKyungpook]{H.~Park,} % 2284
  \author[\instUTokyo]{J.~Park,} % 18203
  \author[\instKISTI]{K.~Park,} % 12243
  \author[\instKEK]{S.-H.~Park,} % 2509
  \author[\instBonn]{B.~Paschen,} % 2159
  \author[\instRomaTreINFN]{A.~Passeri,} % 2116
  \author[\instLouisville]{S.~Patra,} % 3123
  \author[\instTUM]{S.~Paul,} % 2131
  \author[\instLuther]{T.~K.~Pedlar,} % 2421
  \author[\instFrascati]{I.~Peruzzi,} % 2253
  \author[\instHawaii]{R.~Peschke,} % 7123
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{R.~Pestotnik,} % 2476
% \author[\instMelbourne]{F.~Pham,} % 2963
  \author[\instFrascati]{M.~Piccolo,} % 2147
  \author[\instVPI]{L.~E.~Piilonen,} % 2346
% \author[\instTorinoUNIV,\instTorinoINFN]{G.~Pinna~Angioni,} % 13363
  \author[\instUAS]{P.~L.~M.~Podesta-Lerma,} % 2266
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{T.~Podobnik,} % 11223
  \author[\instMississippi]{S.~Pokharel,} % 12283
% \author[\instCPPM]{L.~Polat,} % 9783
% \author[\instTelAviv,\instHSE]{V.~Popov,} % 2096
  \author[\instLMU]{A.~Prakash,} % 21663
  \author[\instKEK]{C.~Praz,} % 2726
  \author[\instISU]{S.~Prell,} % 12743
  \author[\instGiessen]{E.~Prencipe,} % 2219
  \author[\instBonn]{M.~T.~Prim,} % 2501
  \author[\instBINP,\instNSU]{S.~Privalov,} % 12503
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{I.~Prudiiev,} % 19383
% \author[\instSCarolina]{M.~V.~Purohit,} % 2196
  \author[\instHawaii]{H.~Purwar,} % 12363
% \author[\instTUM]{A.~Rabusov,} % 2355
% \author[\instDESY]{N.~Rad,} % 11683
  \author[\instHEPHYVienna]{P.~Rados,} % 7383
  \author[\instHEPHYVienna]{G.~Raeuber,} % 18143
  \author[\instDESY]{S.~Raiz,} % 13003
  \author[\instIITMadras]{V.~Raj,} % 24983
% \author[\instGoettingen]{N.~Rauls,} % 11603
  \author[\instTata]{K.~Ravindran,} % 22503
  \author[\instKrakow]{J.~U.~Rehman,} % 19623
  \author[\instMPP]{M.~Reif,} % 8043
  \author[\instGiessen]{S.~Reiter,} % 2248
  \author[\instBINP,\instNSU]{M.~Remnev,} % 2785
  \author[\instKarlsruhe]{L.~Reuter,} % 16403
  \author[\instWayneState]{D.~Ricalde~Herrmann,} % 9263
  \author[\instIPHC]{I.~Ripp-Baudot,} % 2469
% \author[\instHeidelberg]{M.~Ritzert,} % 2526
  \author[\instPisaUNIV,\instPisaINFN]{G.~Rizzo,} % 2579
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~B.~Rizzuto,} % 3746
  \author[\instUofA,\instIPP]{S.~H.~Robertson,} % 2471
% \author[\instMelbourne]{P.~Rocchetti,} % 13763
% \author[\instUAS]{D.~Rodr\'{i}guez~P\'{e}rez,} % 2176
% \author[\instDESY]{M.~Roehrken,} % 11883
  \author[\instVictoria,\instIPP]{J.~M.~Roney,} % 2244
% \author[\instSCarolina]{C.~Rosenfeld,} % 2082
  \author[\instDESY]{A.~Rostomyan,} % 2481
  \author[\instDESY]{N.~Rout,} % 2965
% \author[\instKrakow]{M.~Rozanska,} % 2205
% \author[\instNapoliUNIV,\instNapoliINFN]{G.~Russo,} % 2388
% \author[\instISU]{D.~Sahoo,} % 2110
% \author[\instKEK,\instSOKENDAI]{Y.~Sakai,} % 2175
% \author[\instRomaTreUNIV,\instRomaTreINFN]{L.~Salutari,} % 17423
% \author[\instUNAM]{G.~Sanchez,} % 2943
  \author[\instMississippi]{D.~A.~Sanders,} % 2458
  \author[\instIITHyderabad]{S.~Sandilya,} % 2286
% \author[\instCincinnati]{A.~Sangal,} % 2384
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{L.~Santelj,} % 2185
% \author[\instIPHC]{C.~Santos,} % 23743
% \author[\instTohoku]{T.~Sanuki,} % 6783
% \author[\instKEK]{Y.~Sato,} % 5243
  \author[\instPittsburgh]{V.~Savinov,} % 2292
  \author[\instUppsala]{B.~Scavino,} % 2518
% \author[\instLMU,\instMPP]{C.~Schmitt,} % 15063
  \author[\instBonn]{J.~Schmitz,} % 12863
  \author[\instDuke]{S.~Schneider,} % 16803
  \author[\instIFIC]{G.~Schnell,} % 12204
% \author[\instKarlsruhe]{M.~Schnepf,} % 15683
% \author[\instUppsala]{K.~Schoenning,} % 22023
% \author[\instHawaii]{J.~Schueler,} % 2824
  \author[\instHEPHYVienna]{C.~Schwanda,} % 2108
% \author[\instCincinnati]{A.~J.~Schwartz,} % 2162
% \author[\instGoettingen]{B.~Schwenker,} % 2405
% \author[\instGoettingen]{M.~Schwickardi,} % 14743
% \author[\instRIKENBNL]{R.~Seidl,} % 26923
  \author[\instNiigata]{Y.~Seino,} % 2517
  \author[\instRomaTreINFN]{A.~Selce,} % 9043
  \author[\instYamagata]{K.~Senyo,} % 2987
  \author[\instCPPM]{J.~Serrano,} % 12124
  \author[\instMelbourne]{M.~E.~Sevior,} % 2328
  \author[\instMainz]{C.~Sfienti,} % 2214
  \author[\instHUNNU]{W.~Shan,} % 11943
% \author[\instIHEPRussia]{M.~Shapkin,} % 2460
% \author[\instMNITJaipur]{C.~Sharma,} % 11584
  \author[\instIITMadras]{G.~Sharma,} % 18423
% \author[\instHawaii]{V.~Shebalin,} % 2339
  \author[\instFudan]{C.~P.~Shen,} % 2464
  \author[\instUTokyo]{X.~D.~Shi,} % 18843
% \author[\instToho]{H.~Shibuya,} % 2234
  \author[\instMcGill]{T.~Shillington,} % 7983
  \author[\instUTokyo]{T.~Shimasaki,} % 16263
% \author[\instNaraWu]{M.~Shimomura,} % 2112
  \author[\instNTUTaiwan]{J.-G.~Shiu,} % 2412
  \author[\instBINP,\instNSU]{D.~Shtol,} % 9223
% \author[\instBINP,\instNSU]{B.~Shwartz,} % 2122
  \author[\instHawaii]{A.~Sibidanov,} % 2419
  \author[\instKarlsruhe]{F.~Simon,} % 2164
  \author[\instPanjab,\instUPES]{J.~B.~Singh,} % 2903
% \author[\instHawaii]{R.~Sinha,} % 3423
  \author[\instMPP,\instTUM]{J.~Skorupa,} % 12523
% \author[\instMelbourne]{K.~Smith,} % 2243
  \author[\instVictoria,\instIPP]{R.~J.~Sobie,} % 2472
  \author[\instMainz]{M.~Sobotzik,} % 8604
  \author[\instTelAviv]{A.~Soffer,} % 2217
  \author[\instIHEPRussia]{A.~Sokolov,} % 2521
% \author[\instDESY]{Y.~Soloviev,} % 2479
  \author[\instBINP]{E.~Solovieva,} % 2398
  \author[\instJLU]{W.~Song,} % 22863
  \author[\instTorinoUNIV,\instTorinoINFN]{S.~Spataro,} % 2117
  \author[\instMainz]{B.~Spruck,} % 2493
% \author[\instNovaGorica]{S.~Stani\v{c},} % 3383
  \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{M.~Stari\v{c},} % 2326
  \author[\instIPHC]{P.~Stavroulakis,} % 20643
  \author[\instBonn]{S.~Stefkova,} % 8783
% \author[\instHawaii]{L.~Stoetzer,} % 19283
% \author[\instVPI]{Z.~S.~Stottler,} % 2267
  \author[\instPadovaUNIV,\instPadovaINFN]{R.~Stroili,} % 2465
% \author[\instPNNL]{J.~Strube,} % 2451
% \author[\instNTUTaiwan]{J.~Su,} % 16623
  \author[\instNagoya]{Y.~Sue,} % 2085
% \author[\instUTokyo]{R.~Sugiura,} % 4644
  \author[\instRCNP,\instGifu]{M.~Sumihama,} % 4243
  \author[\instKEK,\instSOKENDAI,\instNaraWu]{K.~Sumisawa,} % 2583
% \author[\instBonn]{W.~Sutcliffe,} % 3784
  \author[\instChula]{N.~Suwonjandee,} % 14063
% \author[\instKEK,\instSOKENDAI]{S.~Y.~Suzuki,} % 2496
  \author[\instDESY]{H.~Svidras,} % 11783
  \author[\instDESY]{M.~Takahashi,} % 2467
  \author[\instSPU,\instJPARC,\instRIKENMSL]{M.~Takizawa,} % 2437
  \author[\instTorinoINFN]{U.~Tamponi,} % 2366
% \author[\instKEK,\instSOKENDAI]{S.~Tanaka,} % 2530
  \author[\instJAEA]{K.~Tanida,} % 3803
% \author[\instUTokyo]{H.~Tanigawa,} % 2237
% \author[\instKEK]{N.~Taniguchi,} % 2285
  \author[\instPisaUNIV,\instPisaINFN]{F.~Tenchini,} % 2546
% \author[\instOsakaMetropolitan]{Y.~Teramoto,} % 26063
% \author[\instTorinoUNIV,\instTorinoINFN]{F.~Testa,} % 14844
  \author[\instCPPM]{A.~Thaller,} % 16044
  \author[\instMPP]{O.~Tittel,} % 8663
  \author[\instTata]{R.~Tiwary,} % 10403
% \author[\instTriesteINFN]{D.~Tonelli,} % 4564
  \author[\instPadovaINFN]{E.~Torassa,} % 2556
% \author[\instSydney]{N.~Toutounji,} % 2263
  \author[\instTYL]{K.~Trabelsi,} % 2369
  \author[\instBonn]{I.~Tsaklidis,} % 13443
% \author[\instKEK,\instSOKENDAI]{T.~Tsuboyama,} % 2361
% \author[\instNagoya]{N.~Tsuzuki,} % 2352
% \author[\instTitech]{M.~Uchida,} % 2370
  \author[\instKEK,\instSOKENDAI]{I.~Ueda,} % 2519
% \author[\instKEK,\instSOKENDAI]{S.~Uehara,} % 2586
% \author[\instUTokyo]{Y.~Uematsu,} % 5883
% \author[\instLMU]{E.~Uenlue,} % 22283
  \author[\instHSE]{T.~Uglov,} % 2252
  \author[\instKarlsruhe]{K.~Unger,} % 9463
  \author[\instHanyang]{Y.~Unno,} % 2420
  \author[\instKEK]{K.~Uno,} % 14963
  \author[\instKEK,\instSOKENDAI]{S.~Uno,} % 2149
  \author[\instMelbourne]{P.~Urquijo,} % 2302
  \author[\instKEK,\instUTokyo,\instSOKENDAI]{Y.~Ushiroda,} % 2317
% \author[\instBINP,\instNSU]{Y.~V.~Usov,} % 5003
  \author[\instHawaii]{S.~E.~Vahsen,} % 2251
  \author[\instKarlsruhe]{R.~van~Tonder,} % 2706
  \author[\instSydney]{K.~E.~Varvell,} % 2545
  \author[\instISU]{M.~Veronesi,} % 20723
  \author[\instBINP,\instNSU]{A.~Vinokurova,} % 2289
  \author[\instIITHyderabad]{V.~S.~Vismaya,} % 16063
  \author[\instTriesteUNIV,\instTriesteINFN]{L.~Vitale,} % 2415
  \author[\instIFIC]{V.~Vobbilisetti,} % 7364
  \author[\instPerugiaUNIV,\instPerugiaINFN]{R.~Volpe,} % 20183
  \author[\instDuke]{A.~Vossen,} % 2249
% \author[\instMPP,\instTUM]{B.~Wach,} % 8203
% \author[\instMelbourne]{E.~Waheed,} % 2226
  \author[\instUBC]{M.~Wakai,} % 3583
% \author[\instMcGill]{H.~M.~Wakeling,} % 3664
  \author[\instMPP]{S.~Wallner,} % 20363
% \author[\instMalaya]{W.~Wan~Abdullah,} % 2280
% \author[\instCincinnati]{B.~Wang,} % 2569
% \author[\instPittsburgh]{E.~Wang,} % 10983
% \author[\instShandong]{L.~Wang,} % 22443
  \author[\instNTUTaiwan]{M.-Z.~Wang,} % 2074
% \author[\instFudan]{X.~L.~Wang,} % 2076
% \author[\instUTokyo]{Z.~Wang,} % 15743
  \author[\instMcGill]{A.~Warburton,} % 2347
  \author[\instNiigata]{M.~Watanabe,} % 2309
  \author[\instCincinnati]{S.~Watanuki,} % 6843
% \author[\instBonn]{M.~Welsch,} % 7023
% \author[\instTriesteINFN]{O.~Werbycka,} % 6123
  \author[\instDESY]{C.~Wessel,} % 2100
% \author[\instKrakow]{J.~Wiechczynski,} % 2604
% \author[\instMPP]{H.~Windel,} % 2081
  \author[\instKoreaUnivKU]{E.~Won,} % 2410
% \author[\instShandong]{Y.~Xie,} % 20383
  \author[\instSoochow]{X.~P.~Xu,} % 4923
% \author[\instUTokyo]{Z.~Xu,} % 27103
  \author[\instSydney]{B.~D.~Yabsley,} % 3645
  \author[\instKEK]{S.~Yamada,} % 2492
% \author[\instTohoku]{H.~Yamamoto,} % 2964
  \author[\instUSTC]{W.~Yan,} % 2094
% \author[\instZZU]{W.~C.~Yan,} % 2183
  \author[\instKoreaUnivKU]{S.~B.~Yang,} % 2374
  \author[\instFlorida]{J.~Yelton,} % 2067
  \author[\instNankai]{J.~H.~Yin,} % 2365
% \author[\instIHEPChina]{Y.~M.~Yook,} % 2453
  \author[\instHawaii]{K.~Yoshihara,} % 12663
% \author[\instLMU]{B.~Yu,} % 15563
  \author[\instIHEPChina]{C.~Z.~Yuan,} % 2088
  \author[\instJLU]{J.~Yuan,} % 23423
% \author[\instNiigata]{Y.~Yusa,} % 2357
  \author[\instRomaTreUNIV,\instRomaTreINFN]{L.~Zani,} % 2529
  \author[\instIPMU]{F.~Zeng,} % 22043
  \author[\instMETU]{M.~Zeyrek,} % 4023
  \author[\instHawaii]{B.~Zhang,} % 11663
% \author[\instIHEPChina]{J.~Z.~Zhang,} % 2349
% \author[\instFudan]{Y.~Zhang,} % 3303
% \author[\instUSTC]{Z.~Zhang,} % 5363
% \author[\instIHEPChina]{J.~Zhao,} % 3343
  \author[\instBINP,\instNSU]{V.~Zhilich,} % 4703
  \author[\instFudan]{J.~S.~Zhou,} % 12463
  \author[\instShandong]{Q.~D.~Zhou,} % 7323
% \author[\instLNNU]{X.~Y.~Zhou,} % 2380
  \author[\instJLU]{L.~Zhu,} % 25143
% \author[\instLjubljanaUniLJ,\instLjubljanaJSI]{V.~I.~Zhukova,} % 2387
% \author[\instBINP,\instNSU]{V.~Zhulanov,} % 4983
  \author[\instTriesteINFN]{R.~\v{Z}leb\v{c}\'{i}k} % 13403
% \author[\instFudan]{S.~Zou} % 19363
\affiliation[\instCPPM]{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\affiliation[\instYerevan]{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
%%%\affiliation[\instGoettingen]{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\affiliation[\instBeihang]{Beihang University, Beijing 100191, China}
\affiliation[\instBNL]{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\affiliation[\instBINP]{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
%%%\affiliation[\instCMU]{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\affiliation[\instCinvestavIPN]{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\affiliation[\instPrague]{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\affiliation[\instChiangMai]{Chiang Mai University, Chiang Mai 50202, Thailand}
%%%\affiliation[\instChiba]{Chiba University, Chiba 263-8522, Japan}
\affiliation[\instChonnam]{Chonnam National University, Gwangju 61186, South Korea}
\affiliation[\instChula]{Chulalongkorn University, Bangkok 10330, Thailand}
\affiliation[\instCAU]{Chung-Ang University, Seoul 06974, South Korea}
\affiliation[\instConacyt]{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\affiliation[\instDESY]{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\affiliation[\instDuke]{Duke University, Durham, North Carolina 27708, U.S.A.}
\affiliation[\instITAR]{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\affiliation[\instFuJen]{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\affiliation[\instFudan]{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\affiliation[\instGifu]{Gifu University, Gifu 501-1193, Japan}
\affiliation[\instSOKENDAI]{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\affiliation[\instMainz]{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\affiliation[\instGyeongsang]{Gyeongsang National University, Jinju 52828, South Korea}
\affiliation[\instHanyang]{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
%%%\affiliation[\instHeidelberg]{Heidelberg University, 68131 Mannheim, Germany}
\affiliation[\instHNU]{Henan Normal University, Xinxiang 453007, China}
\affiliation[\instKEK]{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\affiliation[\instJPARC]{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
%%%\affiliation[\instHiroshima]{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\affiliation[\instHUNNU]{Hunan Normal University, Changsha 410081, China}
\affiliation[\instFrascati]{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\affiliation[\instNapoliINFN]{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\affiliation[\instPadovaINFN]{INFN Sezione di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaINFN]{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaINFN]{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreINFN]{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoINFN]{INFN Sezione di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteINFN]{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIISc]{Indian Institute of Science, Bengaluru 560012, India}
%%%\affiliation[\instIISER]{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\affiliation[\instIITBhubaneswar]{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\affiliation[\instIITGuwahati]{Indian Institute of Technology Guwahati, Assam 781039, India}
\affiliation[\instIITHyderabad]{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\affiliation[\instIITJodhpur]{Indian Institute of Technology Jodhpur, Jodhpur 342030, India}
\affiliation[\instIITMadras]{Indian Institute of Technology Madras, Chennai 600036, India}
\affiliation[\instIndiana]{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\affiliation[\instIHEPRussia]{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\affiliation[\instHEPHYVienna]{Institute of High Energy Physics, Vienna 1050, Austria}
\affiliation[\instIHEPChina]{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\affiliation[\instIPP]{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\affiliation[\instIOP]{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\affiliation[\instIFIC]{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\affiliation[\instISU]{Iowa State University, Ames, Iowa 50011, U.S.A.}
\affiliation[\instJAEA]{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\affiliation[\instJLU]{Jilin University, Changchun 130012, China}
\affiliation[\instKarlsruhe]{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\affiliation[\instKitasato]{Kitasato University, Sagamihara 252-0373, Japan}
\affiliation[\instKISTI]{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\affiliation[\instKoreaUnivKU]{Korea University, Seoul 02841, South Korea}
%%%\affiliation[\instKSU]{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\affiliation[\instKyotoU]{Kyoto University, Kyoto 606-8501, Japan}
%%%\affiliation[\instKyungpook]{Kyungpook National University, Daegu 41566, South Korea}
%%%\affiliation[\instLNNU]{Liaoning Normal University, Dalian 116029, China}
\affiliation[\instGiessen]{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\affiliation[\instLuther]{Luther College, Decorah, Iowa 52101, U.S.A.}
\affiliation[\instMNITJaipur]{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\affiliation[\instLMU]{Ludwig Maximilians University, 80539 Munich, Germany}
\affiliation[\instMcGill]{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\affiliation[\instMETU]{Middle East Technical University, 06531 Ankara, Turkey}
%%%\affiliation[\instMEPhI]{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\affiliation[\instNagoya]{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNagoyaKMI]{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\affiliation[\instNankai]{Nankai University, Tianjin 300071, China}
\affiliation[\instNaraWu]{Nara Women's University, Nara 630-8506, Japan}
%%%\affiliation[\instUNAM]{National Autonomous University of Mexico, Mexico City, Mexico}
\affiliation[\instHSE]{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\affiliation[\instNTUTaiwan]{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\affiliation[\instKrakow]{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\affiliation[\instNiigata]{Niigata University, Niigata 950-2181, Japan}
\affiliation[\instNSU]{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\affiliation[\instOsakaMetropolitan]{Osaka Metropolitan University, Osaka 558-8585, Japan}
\affiliation[\instRCNP]{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\affiliation[\instPNNL]{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\affiliation[\instPanjab]{Panjab University, Chandigarh 160014, India}
\affiliation[\instMPP]{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
%%%\affiliation[\instMPGHLL]{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\affiliation[\instPanjabPAU]{Punjab Agricultural University, Ludhiana 141004, India}
%%%\affiliation[\instRIKENBNL]{RIKEN BNL Research Center, Upton, New York 11973, U.S.A., U.S.A.}
\affiliation[\instRIKENMSL]{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
%%%\affiliation[\instSeoul]{Seoul National University, Seoul 08826, South Korea}
\affiliation[\instShandong]{Shandong University, Jinan 250100, China}
\affiliation[\instKyiv]{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\affiliation[\instSPU]{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\affiliation[\instSoochow]{Soochow University, Suzhou 215006, China}
\affiliation[\instSoongsil]{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\affiliation[\instSEU]{Southeast University, Nanjing 211189, China}
\affiliation[\instLjubljanaJSI]{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\affiliation[\instSKKU]{Sungkyunkwan University, Suwon 16419, South Korea}
\affiliation[\instTata]{Tata Institute of Fundamental Research, Mumbai 400005, India}
\affiliation[\instTUM]{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\affiliation[\instTelAviv]{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\affiliation[\instToho]{Toho University, Funabashi 274-8510, Japan}
%%%\affiliation[\instTohoku]{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
%%%\affiliation[\instTitech]{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
%%%\affiliation[\instTokyoMetropolitan]{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\affiliation[\instUAS]{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\affiliation[\instNapoliUNIV]{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\affiliation[\instPadovaUNIV]{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\affiliation[\instPerugiaUNIV]{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\affiliation[\instPisaUNIV]{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\affiliation[\instRomaTreUNIV]{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\affiliation[\instTorinoUNIV]{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\affiliation[\instTriesteUNIV]{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\affiliation[\instIJCLab]{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\affiliation[\instIPHC]{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\affiliation[\instAdelaide]{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\affiliation[\instUofA]{University of Alberta, Edmonton, Alberta, T6G 2E1, Canada}
\affiliation[\instBonn]{University of Bonn, 53115 Bonn, Germany}
\affiliation[\instUBC]{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\affiliation[\instCincinnati]{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\affiliation[\instFlorida]{University of Florida, Gainesville, Florida 32611, U.S.A.}
\affiliation[\instHamburg]{University of Hamburg, 20148 Hamburg, Germany}
\affiliation[\instHawaii]{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\affiliation[\instLjubljanaUniLJ]{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\affiliation[\instLouisville]{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
%%%\affiliation[\instMalaya]{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\affiliation[\instManitoba]{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\affiliation[\instLjubljanaUM]{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\affiliation[\instMelbourne]{School of Physics, University of Melbourne, Victoria 3010, Australia}
\affiliation[\instMississippi]{University of Mississippi, University, Mississippi 38677, U.S.A.}
%%%\affiliation[\instUOM]{University of Miyazaki, Miyazaki 889-2192, Japan}
%%%\affiliation[\instNovaGorica]{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\affiliation[\instUPES]{University of Petroleum and Energy Studies, Dehradun 248007, India}
\affiliation[\instPittsburgh]{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\affiliation[\instUSTC]{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\affiliation[\instSAlabama]{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
%%%\affiliation[\instSCarolina]{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\affiliation[\instSydney]{School of Physics, University of Sydney, New South Wales 2006, Australia}
\affiliation[\instTabuk]{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\affiliation[\instUTokyo]{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\affiliation[\instEri]{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\affiliation[\instIPMU]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\affiliation[\instVictoria]{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\affiliation[\instUppsala]{Uppsala University, SE-751 05 Uppsala, Sweden}
\affiliation[\instVPI]{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\affiliation[\instWayneState]{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\affiliation[\instXavier]{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\affiliation[\instXJTU]{Xi'an Jiaotong University, Xi'an 710049, China}
\affiliation[\instYamagata]{Yamagata University, Yamagata 990-8560, Japan}
\affiliation[\instYonsei]{Yonsei University, Seoul 03722, South Korea}
\affiliation[\instTYL]{Toshiko Yuasa Laboratory, Tsukuba 305-0801, Japan}
%%%\affiliation[\instZZU]{Zhengzhou University, Zhengzhou 450001, China}

